Using Auxiliary Data to Boost Precision in the Analysis of A/B Tests on an Online Educational Platform: New Data and New Results

Randomized A/B tests within online learning platforms represent an exciting direction in learning sciences. With minimal assumptions, they allow causal effect estimation without confounding bias and exact statistical inference even in small samples. However, often experimental samples and/or treatment effects are small, A/B tests are underpowered, and effect estimates are overly imprecise. Recent methodological advances have shown that power and statistical precision can be substantially boosted by coupling design-based causal estimation to machine-learning models of rich log data from historical users who were not in the experiment. Estimates using these techniques remain unbiased and inference remains exact without any additional assumptions. This paper reviews those methods and applies them to a new dataset including over 250 randomized A/B comparisons conducted within ASSISTments, an online learning platform. We compare results across experiments using four novel deep-learning models of auxiliary data and show that incorporating auxiliary data into causal estimates is roughly equivalent to increasing the sample size by 20\% on average, or as much as 50-80\% in some cases, relative to t-tests, and by about 10\% on average, or as much as 30-50\%, compared to cutting-edge machine learning unbiased estimates that use only data from the experiments. We show that the gains can be even larger for estimating subgroup effects, hold even when the remnant is unrepresentative of the A/B test sample, and extend to post-stratification population effects estimators.

==> notation.tex <==
\newcommand{\EE}{\mathbb{E}}


\newcommand{\rct}{RCT}
\newcommand{\rem}{REM}
\newcommand{\pop}{POP}%\mathcal{P}}


\newcommand{\pate}[1][\pop]{\EE_{#1}[\tau]}
\newcommand{\sate}[1][\rct]{\overline{\tau}_{#1}}
\newcommand{\patesub}[2][\pop]{\EE_{#1}[\tau\mid #2]}

\newcommand{\tdm}{\hat{\tau}^{DM}}

\newcommand{\alg}{\predr[(0)]{\cdot;\bm{\beta}}}

\newcommand{\rebar}{\hat{\tau}_{rebar}}
\newcommand{\myloop}{\hat{\tau}_{LOOP}(\bm{x})}
\newcommand{\reloop}[1][\predri[],\bm{x}]{\hat{\tau}_{LOOP}(#1)}

\newcommand{\yc}{y(0)}
\newcommand{\yt}{y(1)}
\newcommand{\yci}{y_i(0)}
\newcommand{\yti}{y_i(1)}
\newcommand{\yzi}{y_i(z)}

\newcommand{\pred}[2]{\widehat{y(#1)}\left(#2\right)}
\newcommand{\predic}{\widehat{\yci}}
\newcommand{\predit}{\widehat{\yti}}
\newcommand{\prediz}{\widehat{\yzi}}
\newcommand{\predr}[2][]{\hat{y}^r#1\left(#2\right)}
\newcommand{\predri}[1][i]{\hat{y}_{#1}^r}



==> notes.tex <==
clarify 2 different imputation models--remnant based and within sample

define "within sample" and "remnant based" 

discuss 84 experiments -> 68 experiments -> 227 randomized contrasts



==> to_do.tex <==
\section*{Response to Reviewers}

We are grateful to all three reviewers and to the editors for their careful consideration of our work and their helpful suggestions.

The current revision includes three major changes:
\begin{enumerate}
    \item Following suggestions of reviewers 1 \& 2, we added some important details to Section \ref{sec:imputation}---specifically, a description of how hyperparameters were chosen, the role of dropout, and a note about the possible consequences of a sub-optimal model.
    \item Following suggestions of reviewers 1 \& 2, we added a substantial section at the end of the paper (\S~\ref{sec:limitations}) describing limitations of both the methods we discussed and of our results themselves, along with some comments on how future research may address some of these limitations.
    \item After submitting the first version, we discovered that Figure \ref{fig:ps} contained the wrong plot. We have substituted the correct plot in its place, which corresponds with the discussion in the text. 
\end{enumerate}

We also made a number of smaller changes, mostly regarding grammar, style, and formatting. Several of these were in response to reviewers' suggestions, which we will note below.

\subsection*{Reviewer 1}
\begin{enumerate}
    \item 
        \begin{quote}
        If I understand it correctly, there are two dropout layers in each model with a dropout rate of 50\%. But considering the number of training samples you have and that you are using LSTMs, two 50\% seems too severe (may underfitting? I might be wrong). Have you plotted the learning curves and attempted other hyper-parameters? Though it's not the main focus of the paper, it may tell us what is the best performance (empirically) that the method can achieve.

        You are optimizing the sum of the binary cross-entropy loss and mean squared error. You mentioned that a weight of 16 was applied to the binary cross-entropy loss (which is in the right direction), and optimizing two losses together can improve the ability to predict completion. But the models are bad at predicting problems to mastery. It might be good to try some other methods for balancing the losses in multi-task learning, instead of using a fixed weight. Again, I understand it's not the main focus of the paper, but it would be meaningful to know what is the best performance that the method can achieve.
        \end{quote}
        
        \textbf{Response}: The dropout frequency and the binary cross-entropy loss were both chosen following a grid search and cross-validation, as is now described in the paper in Section \ref{sec:imputation}, following your suggestion. We agree that other methods for balancing the losses may have resulted in better performance. However, having already used the imputation model described to analyze the experiments in the paper, we felt that modifying the model to get better results may compromise our scientific objectivity. That said, it would certainly be interesting to see if a different model performed substantially better. We hope that you and/or other researchers may want to try your hand at it, and we have posted the data at \url{https://osf.io/k8ph9/?view\_only=ca7495965ba047e5a9a478aaf4f3779e}.
        In any event, as we wrote in our revision, our method does not assume that the imputation is optimal, and its estimates remain unbiased with suboptimal models. 

        \item \begin{quote}
            It would be better to have more description of the limitations. I think the authors should include a section/subsection for the limitations of their studies. That will greatly increase the value of the paper. \dots

            However, I think it would be good to mention the limitations of their study. It would also be good to suggest some future work, if possible. This would increase the value of this paper
        \end{quote}
        \textbf{Response}: Thank you for this helpful suggestion. We added an extensive discussion of limitations and future work to the paper (\S~\ref{sec:limitations}), including discussions of limits on the applicability of the the method, costs involved in implementing it (along with the need for more information on potential rewards), risks involved when sample sizes are small, and limits on the conclusions that may be drawn from our case-studies. For each limitation, we also mentioned a direction of future research to solve or ameliorate the problem.
        \item ``Fig 2, Table 2, and Fig 6 are missing periods at the end of the captions.'' Thank you, we have corrected those mistakes.
        
\end{enumerate}

\subsection*{Reviewer 2}

\begin{enumerate}
    \item 
    \begin{quote}
    There’s a lack of thorough discussion on the limitations despite the authors mentioning that the method can impair the precision when subgroups are smaller than 100 in sample size. More about limitations can be provided as discussions.
\end{quote}
\textbf{Response}: (same as to Reviewer 1) Thank you for this helpful suggestion. We added an extensive discussion of limitations and future work to the paper (\S~\ref{sec:limitations}), including discussions of limits on the applicability of the the method, costs involved in implementing it (along with the need for more information on potential rewards), risks involved when sample sizes are small, and limits on the conclusions that may be drawn from our case-studies. For each limitation, we also mentioned a direction of future research to solve or ameliorate the problem.
\item \begin{enumerate}
    \item Page 2, “In general A/B …” $\rightarrow$ “In general,”
    \item Page 6, “Our focus is on bias since we it to …” $\rightarrow$ “since we assume it to …”
    \item Page 7, an individual treatment effect
    \end{enumerate}
    \textbf{Response:} Thank you for catching these mistakes! We have corrected them.

\item ``Page 4, I like the example of definitions, very clear!'' \textbf{Response:} Thank you for saying so! 
\item 
\begin{quote} 
Page 6, Why the estimated coefficient on Z and the regression are biased for $\tau_{RCT}$? It might be good to add a sentence to introduce more.
\end{quote}
\textbf{Response:} Thank you for this suggestion. \citeN{freedman}'s result that OLS gives biased effect estimates was, and remains, surprising. We added a small amount of clarification: basically, the bias occurs when the linear model is incorrect. (In a sense, Freedman's result that the bias decreases with $1/n$ even when the linear model is false may be even more surprising!)
\item 
\begin{quote}
It would be ideal for recalling what is $\hat{y}^r$ and the difference to $\hat{y}_i^r$. In addition, It may be good to talk more about how $\hat{y}^r$ can be used as a covariate, maybe it works in the sense of $\hat{y}_i^r$? But in this case, how does remnant data relate to RCT data?
\end{quote}
\textbf{Response}: Thank you for this comment. The problem was actually sloppy notation on our part, which we have attempted to clean up in the revision. Actually, $\hat{y}^r$ and $\hat{y}_i^r$ are conceptually the same---$\hat{y}^r$ was intended to represent the variable in a more abstract sense, while $\hat{y}_i^r$ was its realization for the $i$th subject. In the revision, we introduced and defined the vector $\bm{\hat{y}^r}$ to (mostly) take the place of the ill-defined $\hat{y}^r$. See \eqref{eq:rebar}. 
\item 
\begin{quote}
Page 11, When determining the randomization of sampling as 1/2 for experiments, did you consider cases when sampling is not really random, but dependent on certain covariates, and is unknown to us?
\end{quote}
\textbf{Response}: This is an interesting question. As we described in the revised Section \ref{sec:data}, the E-trials platform was not equipped to run more complex randomized trials at the time the dataset was collected, so sampling dependent on covariates would not have been possible. In general, as we now note in Section \ref{sec:data}, our method applies if randomization probabilities vary between subjects but are known. However, (as we now note in Section \ref{sec:limitations}) randomization designs in which subjects are not randomized independently remain a subject of future work. We also noted that our methods may be extended to observational studies (i.e. cases like you describe, when selection is based on covariates in an unknown way), which is the subject of a current research project of ours. (Stay tuned!)
\item 
\begin{quote}
How were the 20, 60 numbers and other hyper parameters determined? Not well-tuned models may hard the final results. In addition, dropout maybe should not be used for testing and validation.
\end{quote}
\textbf{Response}: As we now discuss in Section \ref{sec:imputation}, tuning parameters were selected following either prior research or a grid search. Dropout was only used in model training, but not in testing or validation. 
\end{enumerate}



